5G NR-Light at Millimeter Waves: Design Guidelines for Mid-Market IoT Use Cases

5th generation (5G) systems have been designed with three main objectives in mind: increasing throughput, reducing latency, and enabling reliable communications. To meet these (often conflicting) constraints, the 3GPP released a set of specifications for 5G NR, one of the main innovations being the support for communications in the millimeter wave (mmWave) bands. However, how to implement lower complexity, energy efficient, mid-market Internet of Things (IoT) applications is still an on-going investigation, currently led by the 3GPP which is extending the NR standard with NR-Light specifications to support devices with reduced capabilities (REDCAP). While REDCAP devices may also operate at mmWaves to improve the network performance, hardware/software simplifications are needed to support balanced and mixed requirements compared to 5G NR systems. In this context, the contributions of this paper are threefold. First, we present some NR-Light use cases for which the support of the mmWave bands is desirable. Second, we describe how 5G NR can be simplified to achieve NR-Light requirements and expectations. Finally, we evaluate via simulation the performance of NR-Light devices operating at mmWaves in an industrial IoT setup, in terms of cost and complexity, throughput, and latency.

==> Figures/bar-plot-vs-redcap-params.tex <==
\begin{tikzpicture}

    \pgfplotsset{every tick label/.append style={font=\scriptsize}}

\pgfplotsset{
tick label style={font=\scriptsize},
label style={font=\scriptsize},
legend  style={font=\scriptsize},
}

    \pgfplotsset{
        legend image code/.code={
            \draw [#1] (0cm, -0.1cm) rectangle (0.4cm,0.4cm);
        },
    }

    %% THROUGHPUT AXIS
    
    % Baseline only
    \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=0pt,
        bar width=0.15,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        % axis line style={white!80!black},
        %legend style={at={(0.5,0.05)}, anchor=south, draw=white!80!black, font=\footnotesize},
        %legend columns=3,
        %tick align=outside,
        %x grid style={white!80!black},
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        ymin=0, ymax=11,
        ytick style={color=white!15!black},
        %yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,1.2}
    ]
    \addplot [preaction={fill, primaryColor}, very thin] coordinates {
        (0.35, 8.24581770076594)
        };
\end{axis}

    % BW
    \begin{axis}[
            ybar,
            bar shift=-50pt,
            bar width=0.15,
            width=\fwidth,
            height=\fheight,
            at={(0\fwidth,0\fheight)},
            scale only axis,
            axis y line*=left,
            % axis line style={white!80!black},
            %legend style={at={(0.5,0.05)}, anchor=south, draw=white!80!black, font=\footnotesize},
            %legend columns=3,
            %tick align=outside,
            %x grid style={white!80!black},
            xlabel style={font=\scriptsize},
            xlabel={},
            xtick align=inside,
            %xmajorticks=false,
            xmin=0.15, xmax=2.5,
            xticklabel style={align=center},
            xtick style={color=white!15!black},
            xtick={0.35, 1, 2},
            xticklabels={{NR-L-Low \\ (Baseline)}, 
                         {Configuration 1}, 
                         {Configuration 2}},
            %y grid style={white!80!black},
            ylabel style={font=\scriptsize},
            ylabel={Throughput [Mbps]},
            ymajorgrids,
            xmajorgrids,
            %ymajorticks=false,
            ymin=0, ymax=11,
            ytick style={color=white!15!black},
            ytick={2.5, 5, 7.5, 10}
            %yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,1.2}
        ]
        \addplot [preaction={fill, primaryColor}, very thin] coordinates {
            (1, 8.25002439300989)
            (2, 7.86459514715495)
            };
    \end{axis}

    % MCS
    \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=-16.66pt,
        bar width=0.15,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        % axis line style={white!80!black},
        %legend style={at={(0.5,0.05)}, anchor=south, draw=white!80!black, font=\footnotesize},
        %legend columns=3,
        %tick align=outside,
        %x grid style={white!80!black},
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        %y grid style={white!80!black},
        %ymajorgrids,
        %ymajorticks=false,
        ymin=0, ymax=11,
    ]
    \addplot [preaction={fill, primaryColor}, very thin] coordinates {
            (1, 8.16142598635792)
            (2, 8.43446579178086)
        };
\end{axis}

    % Num antennas
    \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=16.66pt,
        bar width=0.15,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        % axis line style={white!80!black},
        %legend style={at={(0.5,0.05)}, anchor=south, draw=white!80!black, font=\footnotesize},
        %legend columns=3,
        %tick align=outside,
        %x grid style={white!80!black},
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        %y grid style={white!80!black},
        %ymajorgrids,
        %ymajorticks=false,
        ymin=0, ymax=11,
    ]
    \addplot [preaction={fill, primaryColor}, very thin] coordinates {
        (1, 9.30121433057365)
        (2, 9.86204979818936)
        };
    \end{axis}

    % TX power
    \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=50pt,
        bar width=0.15,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        % axis line style={white!80!black},
        %legend style={at={(0.5,0.05)}, anchor=south, draw=white!80!black, font=\footnotesize},
        %legend columns=3,
        %tick align=outside,
        %x grid style={white!80!black},
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        %y grid style={white!80!black},
        %ymajorgrids,
        %ymajorticks=false,
        ymin=0, ymax=11,
    ]
    \addplot [preaction={fill, primaryColor}, very thin] coordinates {
        (1, 9.37257317512032)
        (2, 9.98595290026055)
        };
    \end{axis}

    %% LATENCY AXIS

     % Baseline only
     \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=0pt,
        bar width=0.07,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        % axis line style={white!80!black},
        %legend style={at={(0.5,0.05)}, anchor=south, draw=white!80!black, font=\footnotesize},
        %legend columns=3,
        %tick align=outside,
        %x grid style={white!80!black},
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        ymin=0, ymax=33,
        ytick style={color=white!15!black},
        %ytick={0, 0.2, 0.5, 0.75, 1}
        %yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,1.2}
    ]
    \addplot [preaction={fill, secondaryColor}, very thin] coordinates {
        (0.35, 24.926070769672)
        };
\end{axis}

    % BW
    \begin{axis}[
        ybar,
        bar shift=-50pt,
        bar width=0.07,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        axis y line*=right,
        % axis line style={white!80!black},
        %legend style={at={(0.5,0.05)}, anchor=south, draw=white!80!black, font=\footnotesize},
        %legend columns=3,
        %tick align=outside,
        %x grid style={white!80!black},
        xlabel style={},
        xlabel={},
        %xtick align=inside,
        xmajorticks=false,
        xmin=0.15, xmax=2.5,
        %xtick style={color=white!15!black},
        %xtick={0.35, 1, 2},
        %xticklabels={{NR}, {Int.te}, {Worst}},
        %y grid style={white!80!black},
        ylabel style={font=\scriptsize},
        ylabel={Latency [ms]},
        %ymajorgrids,
        %xmajorgrids,
        %ymajorticks=false,
        ymin=0, ymax=33,
        ytick style={color=white!15!black},
        ]
        \addplot [preaction={fill, secondaryColor}, very thin, pattern={north east lines},
                  pattern color=black] coordinates {
            (1, 24.5421820832409)
            (2, 22.6181270233416)
            };
    \end{axis}

    % MCS
    \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=-16.66pt,
        bar width=0.07,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        % axis line style={white!80!black},
        %legend style={at={(0.5,0.05)}, anchor=south, draw=white!80!black, font=\footnotesize},
        %legend columns=3,
        %tick align=outside,
        %x grid style={white!80!black},
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        %y grid style={white!80!black},
        %ymajorgrids,
        %ymajorticks=false,
        ymin=0, ymax=33
    ]
    \addplot [preaction={fill, secondaryColor}, very thin, pattern={dots},
    pattern color=black] coordinates {
            (1, 25.2128156992463)
            (2, 25.4587916938308)
        };
\end{axis}

    % Num antennas
    \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=16.66pt,
        bar width=0.07,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        % axis line style={white!80!black},
        %legend style={at={(0.5,0.05)}, anchor=south, draw=white!80!black, font=\footnotesize},
        %legend columns=3,
        %tick align=outside,
        %x grid style={white!80!black},
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        %y grid style={white!80!black},
        %ymajorgrids,
        %ymajorticks=false,
        ymin=0, ymax=33,
    ]
    \addplot [preaction={fill, secondaryColor}, very thin, pattern={crosshatch},
    pattern color=black] coordinates {
        (1, 15.5960420311129)
        (2, 10.445907741513)
        };
    \end{axis}

    % TX power
    \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=50pt,
        bar width=0.07,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        % axis line style={white!80!black},
        %legend style={at={(0.5,0.05)}, anchor=south, draw=white!80!black, font=\footnotesize},
        %legend columns=3,
        %tick align=outside,
        %x grid style={white!80!black},
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        %y grid style={white!80!black},
        %ymajorgrids,
        %ymajorticks=false,
        ymin=0, ymax=33,
    ]
    \addplot [postaction={pattern={horizontal lines}, pattern color=black}, 
              very thin, preaction={fill, secondaryColor}] coordinates {
        (1, 14.5937116577583)
        (2, 10.6157863955618)
        };
    \end{axis}

    % Legend for the colors ~ different metrics
    \begin{axis}[%
            axis line style={draw=none},
            ybar,
            area legend,
            width=\fwidth,
            height=\fheight,
            at={(0\fwidth,0\fheight)},
            scale only axis,
            %bar shift auto,
            % ybar=0.27cm,
            xmin=0.15,
            xmax=2.5,
            ymin=0,
            ymax=10,
            %xtick=data,
            %xticklabels={,,},
            %ylabel={Throughput [Mbit/s]},
            %xlabel style={font=\footnotesize},
            %ylabel style={font=\footnotesize},
            %tick align=inside,
            %tick pos=left,
            %xtick=data,
            %legend cell align={left},
            legend style={at={(0.5, 1.15)}, font=\small, anchor=south, draw=white!15!black, anchor=south, draw=white!15!black, /tikz/every even column/.append style={column sep=0.3cm}},
            axis line style={-},
            %draw=black,
            %enlarge x limits=0.15,
            hide x axis,
            hide y axis,
            xmajorticks=false,
            ymajorticks=false,
            legend columns=2
        ]

        \addplot [preaction={fill, primaryColor}, very thin]
        coordinates {
                (0,0)
            };
        \addlegendentry{Throughput [Mbps]};

        \addplot [preaction={fill, secondaryColor}, very thin]
        coordinates {
                (0,0)
            };
        \addlegendentry{Latency [ms]};
    \end{axis}

    % Legend for the patterns ~ different REDCAP solutions
    \begin{axis}[%
        axis line style={draw=none},
        ybar,
        area legend,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        %bar shift auto,
        % ybar=0.27cm,
        xmin=0.15,
        xmax=2.5,
        ymin=0,
        ymax=10,
        %xtick=data,
        %xticklabels={,,},
        %ylabel={Throughput [Mbit/s]},
        %xlabel style={font=\footnotesize},
        %ylabel style={font=\footnotesize},
        %tick align=inside,
        %tick pos=left,
        %xtick=data,
        %legend cell align={left},
        legend style={at={(0.5, 1.02)}, font=\small, anchor=south, draw=white!15!black, /tikz/every even column/.append style={column sep=0.3cm}},
        axis line style={-},
        %draw=black,
        %enlarge x limits=0.15,
        hide x axis,
        hide y axis,
        xmajorticks=false,
        ymajorticks=false,
        legend columns=4
    ]

    \addplot [preaction={fill, white}, very thin, pattern={north east lines},
    pattern color=black]
    coordinates {
            (0,0)
        };
    \addlegendentry{BW};

    \addplot [preaction={fill, white}, very thin, pattern={dots},
    pattern color=black]
    coordinates {
            (0,0)
        };
    \addlegendentry{Maximum MCS index};

    \addplot [preaction={fill, white}, very thin, pattern={crosshatch},
    pattern color=black]
    coordinates {
            (0,0)
        };
    \addlegendentry{Number of antennas};

    \addplot [preaction={fill, white}, very thin, pattern={horizontal lines},
    pattern color=black]
    coordinates {
            (0,0)
        };
    \addlegendentry{Maximum TX power};
\end{axis}

\end{tikzpicture}


==> Figures/lat-bar-plot-vs-redcap-params.tex <==
\begin{tikzpicture}

    \pgfplotsset{every tick label/.append style={font=\scriptsize}}

\pgfplotsset{
tick label style={font=\scriptsize},
label style={font=\footnotesize},
}

    \pgfplotsset{
        legend image code/.code={
            \draw [#1] (0cm, -0.1cm) rectangle (0.4cm,0.4cm);
        },
    }

    %% LATENCY AXIS

     % Baseline only
     \begin{axis}[
        ybar,
        %axis line style={draw=none},
        bar shift=0pt,
        bar width=0.15,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        ymin=0, ymax=28,
        ytick style={color=white!15!black},
        %yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,1.2}
    ]
    \addplot [preaction={fill, secondaryColor}, very thin] coordinates {
        (0.35, 24.926070769672)
        };
\end{axis}

    % BW
    \begin{axis}[
            ybar,
            bar shift=-25pt,
            bar width=0.15,
            width=\fwidth,
            height=\fheight,
            at={(0\fwidth,0\fheight)},
            scale only axis,
            xlabel style={font=\footnotesize},
            xlabel={},
            xtick align=inside,
            %xmajorticks=false,
            xmin=0.15, xmax=2.5,
            xticklabel style={align=center},
            xtick style={color=white!15!black},
            xtick={0.35, 1, 2},
            xticklabels={{NR-L-Low \\ (Baseline)}, 
                         {Configuration 1}, 
                         {Configuration 2}},
            %y grid style={white!80!black},
            ylabel style={font=\footnotesize},
            ylabel={Average latency [ms]},
            ymajorgrids,
            xmajorgrids,
            %ymajorticks=false,
            ymin=0, ymax=28,
            ytick style={color=white!15!black},
            %ytick={2.5, 5, 7.5, 10}
            %yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,1.2}
        ]
        \addplot [preaction={fill, secondaryColor}] coordinates {
            (1, 24.5421820832409)
            (2, 22.6181270233416)
            };
    \end{axis}

    % MCS
    \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=-8.33pt,
        bar width=0.15,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        %y grid style={white!80!black},
        %ymajorgrids,
        %ymajorticks=false,
        ymin=0, ymax=28,
    ]
    \addplot [preaction={fill, white}, very thin] coordinates {
            (1, 25.2128156992463)
            (2, 25.4587916938308)
        };
\end{axis}

    % Num antennas
    \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=8.33pt,
        bar width=0.15,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        %y grid style={white!80!black},
        %ymajorgrids,
        %ymajorticks=false,
        ymin=0, ymax=28,
    ]
    \addplot [preaction={fill, secondaryColor}, very thin, pattern={dots},
    pattern color=black] coordinates {
        (1, 15.5960420311129)
        (2, 10.445907741513)
        };
    \end{axis}

    % TX power
    \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=25pt,
        bar width=0.15,
        area legend,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        %y grid style={white!80!black},
        %ymajorgrids,
        %ymajorticks=false,
        ymin=0, ymax=28,
    ]
    \addplot [postaction={pattern={north east lines}, pattern color=black}, 
              very thin, preaction={fill, white}] coordinates {
        (1, 14.5937116577583)
        (2, 10.6157863955618)
        };
    \end{axis}

    % Legend for the patterns ~ different REDCAP solutions
    \begin{axis}[%
        axis line style={draw=none},
        ybar,
        area legend,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        %bar shift auto,
        % ybar=0.27cm,
        xmin=0.15,
        xmax=2.5,
        ymin=0,
        ymax=28,
        %legend cell align={left},
        legend style={at={(0.5, 0.98)}, font=\scriptsize, anchor=south, draw=white!15!black, /tikz/every even column/.append style={column sep=0.3cm}},
        axis line style={-},
        %draw=black,
        %enlarge x limits=0.15,
        hide x axis,
        hide y axis,
        xmajorticks=false,
        ymajorticks=false,
        legend columns=2
    ]

        \addplot [preaction={fill, secondaryColor}, very thin]
    coordinates {
            (0,0)
        };
    \addlegendentry{BW};

    \addplot [preaction={fill, white}, very thin]
    coordinates {
            (0,0)
        };
    \addlegendentry{Maximum MCS index};

    \addplot [preaction={fill, secondaryColor}, very thin, pattern={dots},
    pattern color=black]
    coordinates {
            (0,0)
        };
    \addlegendentry{Number of antennas};

    \addplot [preaction={fill, white}, very thin, pattern={north east lines},
    pattern color=black]
    coordinates {
            (0,0)
        };
    \addlegendentry{Maximum TX power};
    \end{axis}

\end{tikzpicture}

==> Figures/thr-bar-plot-vs-redcap-params.tex <==
\begin{tikzpicture}

    \pgfplotsset{every tick label/.append style={font=\scriptsize}}

\pgfplotsset{
tick label style={font=\scriptsize},
label style={font=\footnotesize},
}

    \pgfplotsset{
        legend image code/.code={
            \draw [#1] (0cm, -0.1cm) rectangle (0.4cm,0.4cm);
        },
    }

    %% THROUGHPUT AXIS
    
    % Baseline only
    \begin{axis}[
        ybar,
        %axis line style={draw=none},
        bar shift=0pt,
        bar width=0.15,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        ymin=0, ymax=11,
        ytick style={color=white!15!black},
        %yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,1.2}
    ]
    \addplot [preaction={fill, primaryColor}, very thin] coordinates {
        (0.35, 8.24581770076594)
        };
\end{axis}

    % BW
    \begin{axis}[
            ybar,
            bar shift=-25pt,
            bar width=0.15,
            width=\fwidth,
            height=\fheight,
            at={(0\fwidth,0\fheight)},
            scale only axis,
            xlabel style={font=\footnotesize},
            xlabel={},
            xtick align=inside,
            %xmajorticks=false,
            xmin=0.15, xmax=2.5,
            xticklabel style={align=center},
            xtick style={color=white!15!black},
            xtick={0.35, 1, 2},
            xticklabels={{NR-L-Low \\ (Baseline)}, 
                         {Configuration 1}, 
                         {Configuration 2}},
            %y grid style={white!80!black},
            ylabel style={font=\footnotesize},
            ylabel={Average throughput [Mbps]},
            ymajorgrids,
            xmajorgrids,
            %ymajorticks=false,
            ymin=0, ymax=11,
            ytick style={color=white!15!black},
            ytick={2.5, 5, 7.5, 10}
            %yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,1.2}
        ]
        \addplot [preaction={fill, primaryColor}, very thin] coordinates {
            (1, 8.25002439300989)
            (2, 7.86459514715495)
            };
    \end{axis}

    % MCS
    \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=-8.33pt,
        bar width=0.15,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        %y grid style={white!80!black},
        %ymajorgrids,
        %ymajorticks=false,
        ymin=0, ymax=11,
    ]
    \addplot [preaction={fill, white}, very thin] coordinates {
            (1, 8.16142598635792)
            (2, 8.43446579178086)
        };
\end{axis}

    % Num antennas
    \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=8.33pt,
        bar width=0.15,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        %y grid style={white!80!black},
        %ymajorgrids,
        %ymajorticks=false,
        ymin=0, ymax=11,
    ]
    \addplot [preaction={fill, primaryColor}, pattern={dots}, very thin] coordinates {
        (1, 9.30121433057365)
        (2, 9.86204979818936)
        };
    \end{axis}

    % TX power
    \begin{axis}[
        ybar,
        axis line style={draw=none},
        bar shift=25pt,
        bar width=0.15,
        area legend,
        hide x axis,
        hide y axis,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        xmajorticks=false,
        ymajorticks=false,
        xmin=0.15, xmax=2.5,
        %y grid style={white!80!black},
        %ymajorgrids,
        %ymajorticks=false,
        ymin=0, ymax=11,
    ]
    \addplot [preaction={fill, white}, pattern={north east lines}, very thin] coordinates {
        (1, 9.37257317512032)
        (2, 9.98595290026055)
        };

    \end{axis}

    % Legend axis
    \begin{axis}[%
        axis line style={draw=none},
        ybar,
        area legend,
        width=\fwidth,
        height=\fheight,
        at={(0\fwidth,0\fheight)},
        scale only axis,
        %bar shift auto,
        % ybar=0.27cm,
        xmin=0.15,
        xmax=2.5,
        ymin=0,
        ymax=10,
        legend cell align={left},
        legend style={at={(0.5, 0.98)}, font=\scriptsize, anchor=south, draw=white!15!black, /tikz/every even column/.append style={column sep=0.3cm}},
        axis line style={-},
        %draw=black,
        %enlarge x limits=0.15,
        hide x axis,
        hide y axis,
        xmajorticks=false,
        ymajorticks=false,
        legend columns=2
    ]

    \addplot [preaction={fill, primaryColor}, very thin]
    coordinates {
            (0,0)
        };
    \addlegendentry{BW};

    \addplot [preaction={fill, white}, very thin]
    coordinates {
            (0,0)
        };
    \addlegendentry{Maximum MCS index};

    \addplot [preaction={fill, primaryColor}, very thin, pattern={dots},
    pattern color=black]
    coordinates {
            (0,0)
        };
    \addlegendentry{Number of antennas};

    \addplot [preaction={fill, white}, very thin, pattern={north east lines},
    pattern color=black]
    coordinates {
            (0,0)
        };
    \addlegendentry{Maximum TX power};
\end{axis}

\end{tikzpicture}

